PRIMA: Privacy-Preserving Identity and Access Management at Internet-Scale

The management of identities on the Internet has evolved from the traditional approach (where each service provider stores and manages identities) to a federated identity management system (where the identity management is delegated to a set of identity providers). On the one hand, federated identity ensures usability and provides economic benefits to service providers. On the other hand, it poses serious privacy threats to users as well as service providers. The current technology, which is prevalently deployed on the Internet, allows identity providers to track the user's behavior across a broad range of services. In this work, we propose PRIMA, a universal credential-based authentication system for supporting federated identity management in a privacy-preserving manner. Basically, PRIMA does not require any interaction between service providers and identity providers during the authentication process, thus preventing identity providers to profile users' behavior. Moreover, throughout the authentication process, PRIMA provides a mechanism for controlled disclosure of the users' private information. We have conducted comprehensive evaluations of the system to show the feasibility of our approach. Our performance analysis shows that an identity provider can process 1,426 to 3,332 requests per second when the key size is varied from 1024 to 2048-bit, respectively.

==> crypto.tex <==
\section{Concrete Construction}
\label{sec:crypto}
TODO

==> details.tex <==
\section{Solution Details}
\label{sec:details}
TODO

==> model.tex <==
\section{System Model}
\label{sec:model}
We first identify system entities, assumptions, potential adversaries and possible attacks.

\subsection{Entities}
There are three types of entities in our system:

\begin{itemize}

    \item \textbf{Users:} 
    These are end users who are interested in consuming services provided by service providers. 
    For authentication, they use services provided by identity providers.
    
    \item \textbf{Identity Providers (IdP):}
    An IdP is responsible for issuing (or revoking) credentials to users. These credentials could be issued after an IdP verifies users' attributes, which could be accomplished out-of-band.
    
    \item \textbf{Service Providers (SP):}
    An SP provides services to users provided they are identified (and authorised). The SP trusts on IdP for issuing and managing credentials
    
\end{itemize}

\subsection{Adversary and Attacks}
The main adversary is IdP that is considered honest-but-curious, meaning it is honest to issue or revoke credentials but curious to profile what services are consumed by users.
% We only assume passive attacks and do not cover active attacks by ...
